Energy efficiency: a Lattice Boltzmann study

The energy consumption and the compute performance of a fluid dynamic code have been investigated varying parallelization approach, arithmetic precision and clock speed. The code is based on a Lattice Boltzmann approximation, is written in Fortran and was executed on high-end GPUs of Leonardo Booster supercomputer. Tests were conducted on single server nodes (up to 4 GPUs in parallel). Performance metrics like the number of operations per second and energy consumption are reported, to quantify how smart coding approach and system adjustment can contribute to reduction of energy footprint while keeping the scientific throughput almost unaltered or with acceptable level of degradation. Results indicate that this application can be executed with 20% of energy saving and reduced thermal stress, at the cost of 5% more computing time. The paper presents preliminary conclusions, as it is a first step of a larger study dedicated to energy efficiency at scale.

==> Makefile <==
PROJECT=main

default: obj/$(PROJECT).pdf

display: default
	(${PDFVIEWER} obj/$(PROJECT).pdf &)

### Compilation Flags
PDFLATEX_FLAGS  = -halt-on-error -output-directory obj/

### File Types (for dependancies)
TEX_FILES = $(shell find ./ -name '*.tex' -or -name '*.sty' -or -name '*.cls')
BIB_FILES = $(shell find ./ -name '*.bib')
BST_FILES = $(shell find ./ -name '*.bst')
IMG_FILES = $(shell find ./fig -path '*.jpg' -or -path '*.png' -or \( \! -path './obj/*.pdf' -path '*.pdf' \) )

UNAME := $(shell uname)

ifeq ($(UNAME), Linux)
PDFVIEWER = evince
endif

ifeq ($(UNAME), Darwin)
PDFVIEWER = open
endif
clean:
	rm -rf obj/

obj/:
	mkdir -p obj/

obj/$(PROJECT).aux: $(TEX_FILES) $(IMG_FILES) | obj/
	pdflatex -draftmode $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).bbl: $(BIB_FILES) | obj/$(PROJECT).aux
	bibtex obj/$(PROJECT)
	pdflatex -draftmode $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).pdf: obj/$(PROJECT).aux $(if $(BIB_FILES), obj/$(PROJECT).bbl)
	pdflatex -draftmode $(PDFLATEX_FLAGS) $(PROJECT)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)


==> energy.tex <==
\section{Energy figure for different GPUS}

\begin{table}
    \centering
    \begin{tabular}{|c|c||c|c|} \hline
       Step               &         & ETS      & TTS     \\ \hline \hline
       NVIDIA (Leonardo)  & openacc & 269070   &  212''  \\ \hline
       AMD (Adastra)      & openacc & 110551*4 &  403''    \\ \hline 
       AMD (Adastra)      & offload & 110575*4  &  404''    \\ \hline 
    \end{tabular}
    \caption{ETS, TTS for AMD and NVIDIA GPU (to fix exact test case)}
    \label{Tab:EnergyJU}
\end{table}
\newpage
